SPA: Verbal Interactions between Agents and Avatars in Shared Virtual Environments using Propositional Planning

We present a novel approach for generating plausible verbal interactions between virtual human-like agents and user avatars in shared virtual environments. Sense-Plan-Ask, or SPA, extends prior work in propositional planning and natural language processing to enable agents to plan with uncertain information, and leverage question and answer dialogue with other agents and avatars to obtain the needed information and complete their goals. The agents are additionally able to respond to questions from the avatars and other agents using natural-language enabling real-time multi-agent multi-avatar communication environments. Our algorithm can simulate tens of virtual agents at interactive rates interacting, moving, communicating, planning, and replanning. We find that our algorithm creates a small runtime cost and enables agents to complete their goals more effectively than agents without the ability to leverage natural-language communication. We demonstrate quantitative results on a set of simulated benchmarks and detail the results of a preliminary user-study conducted to evaluate the plausibility of the virtual interactions generated by SPA. Overall, we find that participants prefer SPA to prior techniques in 84\% of responses including significant benefits in terms of the plausibility of natural-language interactions and the positive impact of those interactions.

==> VR2020_arXiv/tex/related_work.tex <==
\section{Related Work}
\label{nlpcrowds:sec:nlp_related}
In this section, we give an overview of relevant work in action-planning, multi-agent simulation, and verbal communication.

\subsection{Action Planning}

Action planning, sometimes referred to as classical planning, task planning, or logical planning in the literature \citep{Russell:2009:AIM:1671238, ghallab2004automated}, deals with constructing a set of actions taken by an intelligent agent to solve a problem or achieve a goal.
Classical approaches such as STRIPS \citep{fikes1971strips}, ADL, \citep{pednault1989adl} and PDDL \citep{fox2003pddl2} construct domain description formalisms which allows many distinct domains to be solvable with a common approach.
Recent work has addressed uncertainty through continual planning \citep{brenner2009continual}, or by encoding sensing actions \citep{petrick2004extending}. 
The latter approach encodes a specific ``sensing'' action for each kind of information the agent may need.
Our approach seeks to minimize explicit sensing actions, instead employing natural-language interactions and generic exploration to resolve uncertainty.
Epistemic planning approaches \citep{eger2018keeping,martens2015ceptre}, typically employed in agent-interaction scenarios, typically solve uncertainty via each agent modeling their perception of the beliefs of other agents in a turn-based interaction.
These models are inherently complimentary to our overall algorithmic approach.
However, it is unclear how an agent would determine the best question to ask given an epistemic model or how ``overhearing'' and indirect communication are modeled in these cases.

\subsection{Human and Single Agent Interactions}

Interactions between humans and automated agents can be subdivided into human-robot interactions (HRI) and human interactions with a digital or virtual agent, also called Embodied Conversational Agents (ECA). 

In the domain of HRI, robots typically plan dialog to clarify a human operator's intentions in a collaborative context~\citep{doshi2008spoken,bisk2016natural}.
The robot does not maintain independent goals or a non operator-centric representation of the domain.
The robot works as a subservient collaborator, typically limited to interaction with a single human operator.
Recent work has demonstrated a robot requesting assistance in a specific collaborative-task \citep{tellex2014asking}. 
Our framework is complimentary to the proposed language model and could be used with such a system for embodied conversation on a physical robot.
Some work has incorporated sensor uncertainty \citep{tenorth2017representations}, but modeling unknown information remains a challenge across domains.
Our approach allows agents to act on their own goals and employ natural-language interactions with multiple avatars or agents by specifying a range of domain information types without fully specifying the agent's knowledge.

Prior work in Embodied Conversation Agents (ECA) has single-agent communication with a human avatar using complex but well-structured dialogue \citep{graesser2014learning}. \citettwo{Rickel and Johnson}{rickel1999virtual} demonstrated positive effects on team training using virtual agents in a mixed agent-avatar environment. In these cases, the agent's behavior is fundamentally user-centric i.e. rather than behaving as an independent entity, the agent's plan revolves around the avatar. 
Some work has demonstrated capabilities in learning from natural language interaction \citep{Wang2016, Thomason2015a}. However, these methods limit the interactions to a single user and do not generalize to unstructured interactions. 

\subsection{Multi-agent Planning}

Action planning for interactive multi-agent systems has typically been limited to locomotion-based actions, and comprises of choosing an appropriate goal position for each agent and computing its trajectory. A large body of research exists on planning paths to an agent's goal \citep{Snook00,tollPLE} and local-avoidance behaviors \citep{ORCA,karamouzas2014universal,Schadschneider01} for agents. Our work is complimentary to these approaches and our agents can use any of these methods for path planning.
However, many of these approaches rely on rigid finite-state machines to generate goals for the agents \citep{curtis2016menge,ulicny2002towards}. Some approaches have been proposed to incorporate contextual interactions \citep{Paris09,Shao05}, but in these cases the behaviors of the agents are pre-encoded and activated when specific conditions are met. 
Instead, our approach allows for dynamically creating action plans for agents without a rigid or pre-encoded structure. 
Our agents generate and execute plans as needed to satisfy diverse goals.
Agents can plan simple goal positions, or complex goals, i.e. interacting with a specific agent or acquiring some item from the environment.

\subsection{Communication in Multi-agent systems}

Some prior work has introduced communication capabilities in multi-agent systems using message-passing or packet-based approaches to model interaction 
\citep{kullu2017acmics}, auditory cues \citep{huang2013spread}, social contagion \citep{chao2010simulation}, or information sharing \citep{Pelechano06}.
In each approach, agents communicate using a strict message structure, or implicitly through the sharing of data and thus preclude the use of interactive verbal communication.
\citettwo{Sun et al.}{sun2012animating} generated animated conversation for agents in a simulated crowd, and \citettwo{Brenner and Kruijff-Korbayova}{brenner2008continual} leveraged message-passing to enable multiple agents to collaborate with a simulated user (i.e. not an actively controlled avatar) in a shared-task.
In each case, the natural-language dialog was generated post-simulation as an animation feature. By contrast, our approach allows the agents to communicate with other agents and avatars using plausible verbal communication in real time. 






==> VR2020_arXiv/tex/user_study_full.tex <==
\subsection{User Evaluation}




This section provides a formal description of the user study we conducted to evaluate the plausibility of agent-avatar interactions and the overall simulation generated as a result of our algorithm. In addition, we provide the complete set of participant responses and additional response analysis.

\textbf{Experiment Goals \& Expectations:} We hypothesize that verbal communication between agents and avatars will enhance the perceived plausibility of the simulation, and generate positive impressions as compared to the control conditions. 

\subsubsection{Comparison Conditions}

\begin{itemize}
	\item \textbf{No Agents}: In the no agents case, a user avatar explores a virtual environment without any virtual agents present.
	\item \textbf{No Communication}: In the no communication case, a user avatar explores a virtual environment with agents who could not interact using natural-language communication.
\end{itemize}
	
\subsubsection{Experimental Design}

 This study was conducted based on a within-subjects, paired-comparison design. 
 Each scenario was displayed with a text-based prompt to provide the appropriate context. 
 Participants were shown two pre-recorded videos of a subject interacting with the system in a side-by-side comparison of our method and one of the comparison methods. 
 They were then asked to answer a short questionnaire before moving on to the next scenario. 
 The order of scenario and the positioning of the methods was counterbalanced. 


\subsubsection{Environments}

The multi-agent tradeshow scenario and multi-agent museum were used in this study.
Three confederates were recruited to participate as the avatar in the environments. 
In trials using our method, the confederate was allowed to interact with the agents using natural-language communication.
In each case, the avatar was piloted from a first-person view. Their interactions were recorded via screen capture and a microphone.

\textbf{Tradeshow}: The avatar was instructed to find the ``registration booth''. They were shown a picture of the booth before beginning their task but were not told its location. In the SPA case, virtual agents in the environment were able to interact and provide the location of the booth to the avatar. We refer the reader to the main document for visual examples of the benchmarks.

\textbf{Museum}: The avatar was instructed to find a specific statue in the museum but was not told the location of the statue. 
The statue in question was Lucy, courtesy of the Stanford University Computer Graphics Laboratory.
In the SPA case, a virtual agent near the avatar's starting position was provided knowledge of the location. 
The avatar was able to ask this agent the location of the statue. 
In addition, two agents were placed along the path to the goal who would interrupt the avatar's progress and ask the avatar for the locations of other statues as they passed.

\subsubsection{Metrics}

Participants were asked a set of common questions for both comparison methods, with specific additions for each comparison method.

\textbf{Common Metrics}: Participants were asked to indicate which simulation more closely reflected a real-world scenario on a Likert scale with 1 indicating strong preference for the method presented on the left, 7 indicating strong preference for the method presented on the right, and 4 indicating no preference. They were then asked the impact of the following items on their preference: the presence of natural language communication, the quality of the verbal responses from the agents, and the quality of the animation. These were answered on a Likert scale with 1 indicating strong negative impact, 7 indicating strong positive impact, and 4 indicating no impact.

\textbf{No Agent Metrics}: Participants were additionally asked what impact the presence of the virtual agents had on their preference. 

\textbf{No Communication Metrics}: Participants were additionally asked which of the methods demonstrated more plausible interactions, in which simulation did the agents appear to benefit more from their interactions with the avatar, and in which simulation did the avatar appear to benefit more from their interactions with the virtual agents.

\subsubsection{Results}


The study was taken by 14 participants. 
We normalized the data for comparative questions such that a response of $1$ indicates strong preference for our method.
We collapsed the common metrics across trials as well as plausibility of interactions question for the No Communication metric and the presence of virtual agents from the No Agents metric.
We performed a one-sample t-test comparing the mean of each question with a hypothetical mean of 4 (no preference or no impact).
We limit our discussion below to questions which directly deal with natural-language interaction and preference for the methods. \Cref{nlpcrowds:table:userstudy_frequency} gives complete details of the participant responses collected for our user evaluation. 

\begin{table*}[t]
	\centering
	\caption{{\bf Performance Benchmark Details}. We detail number of agents, desires, and the NL-I details of the benchmark scenarios including how many questions were asked, statements made, facts overheard by agents, and parser failures. We observe, as expected, that as the number of agents and desires increases, the amount of information gained from overhearing nearby agents increases.}
	\label{nlpcrowds:table:benchmark_details}
	
	\begin{tabular}{llrrrrrr}
		\toprule
		Scene &  Agents &  Desires &  Statements & Questions & Facts Overheard &  
		Parser failures \\
		\midrule
		Anti-podal Circle &    10 &    30 &   14 &   5 &      28  &  0 \\
		Evacuation &  11 &   10 &   4 &  0 &   20 &  0 \\
		Museum &    5 &  9 &   20 &     13 &      3 &      0 \\
		Trade Show &    4 &  1 &    3 &   2 &      0 &      0 \\
		\bottomrule
	\end{tabular}
\end{table*}


We found the question ``Which simulation more closely reflects a real-world scenario'' significant in both the no agents condition 
($t(27)=-6.204, p < 0.000$), 
and the no communication condition 
($t(27)=-7.887, p < 0.000$).
We found the question ``What impact did the presence of natural language interaction have on your answer'' significant in both the no agents condition ($t(27)=10.200, p < 0.000$),
and the no communication condition 
($t(27)=14.925, p < 0.000$).
We found the question ``What impact did the quality of the verbal responses from the agents have on your answer'' significant in both the no agents condition 
($t(27)=5.473, p < 0.000$), 
and the no communication condition
($t(27)=9.218, p < 0.000$).
We found the question ``In which simulation did the interactions between the user and the agents seem more plausible'' significant in the no communication condition 
($t(27)=-6.765, p < 0.000$). 
It was not asked of the no agents condition.
We found the question ``What impact did the presence of virtual agents have on your answer'' significant in the no agents condition 
($t(27)=13.478, p < 0.000$). 
It was not asked of the no communication condition.
perception of the impact of natural language interactions.


\textbf{Analysis:} As detailed in section 6 of the main document, participant responses demonstrate the benefits of our algorithm in terms of generating plausible agent-avatar interactions ($2.46 \pm 1.20$).
In both comparative conditions, either without agents or without communication, participants found our method to generate simulations and interactions with better reflect real-world scenarios ($2.29 \pm 1.15$ and $2.29 \pm 1.46$).

Overall, Participants preferred our approach in 84\% of responses. 
Of those responses, 84\% were strong preferences ($r \leq 2$).
\Cref{nlpcrowds:fig:histogram_preferences_realworld} and \Cref{nlpcrowds:fig:histogram_preferences_nli} provide additional details about our method's advantages over prior approaches.


\begin{figure*}[t]
	\centering
	\begin{tabular}{cc}
	\includegraphics[width=0.49\textwidth]{nlpcrowds/final/planning_v_agents.pdf} &
	\includegraphics[width=0.51\textwidth]{nlpcrowds/final/planning_v_information.pdf} \\
	(A) & (B) 
	\end{tabular}
	\caption{\textbf{Performance Results Varying Number of Agents and Problem Size}: \textbf{(A) Varying agents on a fixed domain size (100 predicates):} We observe that our algorithmic approach's performance scales linearly in the number of agents. \textbf{(B) Varying domain size for a fixed number of agents (10 agents):} We observe that our algorithm's performance scales exponentially in the size of the problem domain. This is consistent with propositional approaches. However, our two stage planning approach enables rapid replanning after the initial planning step, reducing overall planning time.}
	\label{nlpcrowds:fig:performance_macro_graphs}
	\vspace*{-0.1in}
\end{figure*}


\begin{figure*}[t]
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.45\textwidth]{nlpcrowds/final/intent_nlp_dumbagent_q1_closely_reflects.pdf} &
		\includegraphics[width=0.45\textwidth]{nlpcrowds/final/intent_nlp_noagent_q1_closely_reflects.pdf}
		\\
		\textbf{(A)} & \textbf{(B)} 
	\end{tabular}
	\caption{\textbf{Histogram data of user responses for Which scenario better reflects real-world scenarios}: Participants in our evaluation found simulations using SPA significantly more plausible compared to simulations with a prior approach {\bf (A)} and simulations with no agents {\bf (B)}. This indicates that the presence of agents has a positive impact on plausibility and that our agents behave sufficiently well to increase plausibility with respect to agents lacking SPA. }
	\label{nlpcrowds:fig:histogram_preferences_realworld}
\end{figure*}

\begin{figure*}[t]
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.45\textwidth]{nlpcrowds/final/intent_nlp_dumbagent_q4_presence_natural.pdf} &
		\includegraphics[width=0.45\textwidth]{nlpcrowds/final/intent_nlp_noagent_q4_presence_natural.pdf}
		\\
		\textbf{(A)} & \textbf{(B)}
	\end{tabular}
	\caption{\textbf{Histogram data of user responses for impact of natural language interactions} Participants in our evaluation found the presence and quality of the natural language interactions had a significant impact on their preference for our approach to simulations with agents lacking SPA {\bf A} and simulations without agents {\bf b}. In addition, the preference for the quality of the natural language interactions generated with SPA is stronger when compared to agents not able to communicate.}
	\label{nlpcrowds:fig:histogram_preferences_nli}
	\vspace*{-0.1in}
\end{figure*}

\begin{table*}[h]
	\centering
	\caption{{\bf Frequency of Responses in User Evaluation}. This table shows the frequency of participant responses in the user evaluation, as well as the means and p-value for a one-sample t-test with a hypothetical mean of 4. For comparative questions, responses less than 4 indicate preference for our agents. For impact questions, responses greater than 4 indicate positive impacts. We found participant responses to all question significant.}
	\label{nlpcrowds:table:userstudy_frequency}
	\begin{tabular}{lrrrrrrrrrr}
		\toprule
		Question & 1 & 2 & 3 & 4 & 5 & 6 & 7 & mean & std & p-value \\
		\midrule
		\multicolumn{11}{l}{{\bf NL-I Agents vs Non-Interactive Agents }}\\
		\multicolumn{11}{l}{{\bf Comparative Questions (NL-I Agents left) }}\\
		\midrule
		More closely reflects real scenario & 6 & 13 & 7 & 0 & 1 & 1 & 0 & 2.29 & $\pm 1.15$ & $< 0.000$ \\
		Agents benefit more from interaction & 11 & 4 & 1 & 11 & 0 & 1 & 0 & 2.57 & $\pm 1.53$ & $ < 0.000 $ \\
		User benefits more from interaction & 17 & 10 & 0 & 0 & 0 & 1 & 0 & 1.54 & $\pm 1.00$ & $ < 0.000 $ \\
		More plausible interactions & 5 & 13 & 5 & 2 & 3 & 0 & 0 & 2.46 & $\pm 1.20$ & $ < 0.000 $ \\
		\multicolumn{11}{l}{{\bf Impact Questions }}\\
		Presence of natural Language & 0 & 0 & 0 & 1 & 3 & 14 & 10 & 6.18 & $\pm 0.77$ & $ < 0.000 $ \\
		Quality of the verbal interactions & 0 & 0 & 2 & 1 & 3 & 18 & 4 & 5.75 & $\pm 1.00$ & $ < 0.000 $ \\
		Animation of the virtual agents & 0 & 0 & 4 & 13 & 3 & 3 & 5 & 4.74 & $\pm 1.36$ & 0.010 \\
		\midrule
		\multicolumn{11}{l}{{\bf NL-I Agents vs No Agents }}\\
		\multicolumn{11}{l}{{\bf Comparative Questions (NL-I Agents left) }}\\
		\midrule
		More closely reflects real scenario & 9 & 10 & 6 & 1 & 0 & 1 & 1 & 2.29 & $\pm 1.46$ & $ < 0.000 $ \\
		\midrule
		\multicolumn{11}{l}{{\bf Impact Questions }}\\
		\midrule
		Presence of the virtual agents & 0 & 0 & 0 & 0 & 8 & 10 & 10 & 6.07 & $\pm 0.81$ & $ < 0.000 $ \\
		Actions of the virtual agents & 0 & 0 & 0 & 6 & 9 & 10 & 3 & 5.36 & $\pm 0.95$ & $ < 0.000 $ \\
		Presence of natural Language & 0 & 0 & 0 & 3 & 6 & 12 & 7 & 5.82 & $\pm 0.94$ & $ < 0.000 $ \\
		Quality of the verbal interactions & 0 & 1 & 2 & 3 & 7 & 12 & 3 & 5.29 & $\pm 1.24$ & $ < 0.000 $ \\
		Animation of the virtual agents & 0 & 0 & 3 & 11 & 10 & 2 & 2 & 4.61 & $\pm 1.03$ & 0.004 \\
		\bottomrule
	\end{tabular}
\end{table*}


